Tree semantic segmentation from aerial image time series

Earth's forests play an important role in the fight against climate change, and are in turn negatively affected by it. Effective monitoring of different tree species is essential to understanding and improving the health and biodiversity of forests. In this work, we address the challenge of tree species identification by performing semantic segmentation of trees using an aerial image dataset spanning over a year. We compare models trained on single images versus those trained on time series to assess the impact of tree phenology on segmentation performances. We also introduce a simple convolutional block for extracting spatio-temporal features from image time series, enabling the use of popular pretrained backbones and methods. We leverage the hierarchical structure of tree species taxonomy by incorporating a custom loss function that refines predictions at three levels: species, genus, and higher-level taxa. Our findings demonstrate the superiority of our methodology in exploiting the time series modality and confirm that enriching labels using taxonomic information improves the semantic segmentation performance.

==> tables/color_code.tex <==
\begin{table}[htbp]
\centering
\begin{tabular}{ll}
\toprule
\textbf{Common Name (Scientific Name)} & \textbf{Abbreviation} \\
\midrule
Balsa Fir (Abies balsamea) & \colorbox[HTML]{E67E22}{\textcolor{white}{ABBA}} \\
Striped Maple (Acer pensylvanicum) & \colorbox[HTML]{2980B9}{\textcolor{white}{ACPE}} \\
Red Maple (Acer rubrum) & \colorbox[HTML]{8E44AD}{\textcolor{white}{ACRU}} \\
Sugar Maple (Acer saccharum) & \colorbox[HTML]{27AE60}{\textcolor{white}{ACSA}} \\
Maple (Acer Sp.)  & \colorbox[HTML]{F1C40F}{\textcolor{black}{Acer}} \\
Swamp Birch (Betula alleghaniensis) & \colorbox[HTML]{E74C3C}{\textcolor{white}{BEAL}} \\
Paper Birch (Betula papyrifera) & \colorbox[HTML]{1ABC9C}{\textcolor{white}{BEPA}} \\
American Beech (Fagus grandifolia) & \colorbox[HTML]{F39C12}{\textcolor{white}{FAGR}} \\
Tamarack (Larix laricina) & \colorbox[HTML]{9B59B6}{\textcolor{white}{LALA}} \\
Dead Tree & \colorbox[HTML]{16A085}{\textcolor{white}{DEAD}} \\
Spruce (Picea Sp.)  & \colorbox[HTML]{F7DC6F}{\textcolor{black}{Picea}} \\
Eastern White Pine (Pinus strobus) & \colorbox[HTML]{C0392B}{\textcolor{white}{PIST}} \\
Aspen & \colorbox[HTML]{3498DB}{\textcolor{white}{Populus}} \\
Northern White-Cedar (Thuja occidentalis) & \colorbox[HTML]{D35400}{\textcolor{white}{THOC}} \\
Eastern Hemlock (Tsuga canadensis) & \colorbox[HTML]{2C3E50}{\textcolor{white}{TSCA}} \\
\bottomrule
\end{tabular}
\caption{Tree species and their abbreviations. The color corresponding the species is highlighted in the second column and is consistent for all the plots and figures.}
\label{tab:tree-abbreviations}
\end{table}
